Error Bounds of Projection Models in Weakly Supervised 3D Human Pose Estimation

The current state-of-the-art in monocular 3D human pose estimation is heavily influenced by weakly supervised methods. These allow 2D labels to be used to learn effective 3D human pose recovery either directly from images or via 2D-to-3D pose uplifting. In this paper we present a detailed analysis of the most commonly used simplified projection models, which relate the estimated 3D pose representation to 2D labels: normalized perspective and weak perspective projections. Specifically, we derive theoretical lower bound errors for those projection models under the commonly used mean per-joint position error (MPJPE). Additionally, we show how the normalized perspective projection can be replaced to avoid this guaranteed minimal error. We evaluate the derived lower bounds on the most commonly used 3D human pose estimation benchmark datasets. Our results show that both projection models lead to an inherent minimal error between 19.3mm and 54.7mm, even after alignment in position and scale. This is a considerable share when comparing with recent state-of-the-art results. Our paper thus establishes a theoretical baseline that shows the importance of suitable projection models in weakly supervised 3D human pose estimation.

==> chapters/supplementary_material.tex <==
\section{Detailed Derivations}
For the sake of completeness, we provide more detailed derivations for the best-case 3D estimates and the resulting minimal MPJPE under the normalized and weak perspective projection model.

\subsection{Best-Case Normalized Perspective 3D Estimate}
Recall that under the normalized perspective projection, the 3D pose estimate only depends on the per-point depth estimate $\widetilde{Z}_i$.
Under normalization by translation as well as scaling, the squared JPE has the same form, with
\begin{align}
  \Delta d_i^2(\widetilde{Z}_i) &= \left ( \widetilde{Z}_i a - X_i \right)^2 + \left ( \widetilde{Z}_i b - Y_i \right )^2 + \left ( \widetilde{Z}_i - Z_i \right )^2  \nonumber \\
                              &= \widetilde{Z}_i^2 \left ( a^2 + b^2 + 1 \right ) - 2\widetilde{Z}_i \left ( aX_i +bY_i - Z_i \right ) \nonumber \\
                              & \; \; \; \; + X_i^2 + Y_i^2 + Z_i^2 \ ,
\end{align}
where $a$ and $b$ are independent of $\widetilde{Z}_i$. With $\Delta d_i^2$ being a square function in $\widetilde{Z}_i$, 
we obtain the best-case depth estimate by differentiating $\Delta d_i^2$ w.r.t. $\widetilde{Z}_i$:
\begin{equation}
\label{eq:derivative-minimum-distance}
\Delta d_i^{2\prime}(\widetilde{Z}_i) = 2 \cdot \left ( \widetilde{Z}_i \left (a^2 + b^2 + 1\right ) - a X_i - b Y_i - Z_i \right ) \ .
\end{equation}
Setting this expression equal to zero yields the optimal depth estimate $\widetilde{Z}_i^\ast$, with
\begin{align}
\widetilde{Z}_i^\ast & = \frac{a X_i + b Y_i + Z_i}{1 + a^2 + b^2} \ .
\label{eq:z_i-min}
\end{align}

\subsubsection{Minimal JPE under Translation Normalization}
Under normalization by translation, we have $a = \left( \frac{X_i}{Z_i} + dx \left( \frac{1}{Z_i} - \frac{1}{Z} \right) \right )$
and $b =\frac{Y_i}{Z_i}$.
With the optimal 3D estimate $\widetilde{P}_i = (\widetilde{X}_i^\ast, \widetilde{Y}_i^\ast, \widetilde{Z}_i^\ast)$, the resulting minimal JPE for joint $P_i$ is
\begin{align}
\Delta d_i &= 
\sqrt{\left (\widetilde{X}_i^\ast - X_i \right )^2 + \left (\widetilde{Y}_i^\ast - Y_i \right )^2 + \left (\widetilde{Z}_i^\ast - Z_i \right )^2} \nonumber \\
& = \sqrt{\frac{\left (a Y_i - b X_i \right )^2 + \left (a Z_i - X_i \right )^2 + \left (b Z_i - Y_i \right )^2}{1 + a^2 + b^2}} \nonumber \\
& = \sqrt{\frac{dx^2 \cdot \left (\frac{1}{Z_i} - \frac{1}{Z} \right )^2 \cdot \left (Y_i^2 + Z_i^2 \right ) }{1 + a^2 + b^2}} \nonumber \\
\label{eq:minimum-delta-d}
& = \abs{dx \left (\frac{1}{Z_i} - \frac{1}{Z} \right )} \sqrt{\frac{Y_i^2 + Z_i^2}{1 + a^2 + b^2}} \ .
\end{align}

\subsubsection{Minimal JPE under Scale Normalization}
Under normalization by scaling, we have $a = \rho \cdot \frac{X_i}{Z_i + dz}$ and $b = \rho \cdot \frac{Y_i}{Z_i + dz}$.
The resulting minimal JPE for joint $P_i$ is calculated as
\begin{align}
	\Delta d_i &= \sqrt{\left (\widetilde{X}_i^\ast - X_i \right )^2 + \left (\widetilde{Y}_i^\ast - Y_i \right )^2 + \left (\widetilde{Z}_i^\ast - Z_i \right )^2} \nonumber\\
	&=\sqrt{\frac{\left (a Y_i - b X_i \right )^2 + \left (a Z_i - X_i \right )^2 + \left (b Z_i - Y_i \right )^2}{1 + a^2 + b^2}} \nonumber \\ 
	&= \sqrt{\frac{\left (\rho \cdot \frac{X_i}{Z_i + dz}\cdot Z_i - X_i \right )^2 + \left (\rho \cdot \frac{Y_i }{Z_i + dz}\cdot Z_i- Y_i \right )^2}{1 + a^2 + b^2}} \nonumber \\
	&= \sqrt{\frac{\left (X_i^2 \left (\rho \cdot \frac{Z_i}{Z_i + dz} - 1 \right) \right )^2 + \left (Y_i^2 \left (\rho \cdot \frac{Z_i}{Z_i + dz}-1 \right ) \right )^2}{1 + a^2 + b^2}} \nonumber \\
	&= \abs{1 - \rho \cdot \frac{Z_i}{Z_i + dz}}  \sqrt{\frac{X_i^2 + Y_i^2}{1 + a^2 + b^2}} \ .
\end{align}

\begin{figure*}[t]
  \centering
  \includegraphics[width=0.80\linewidth]
                   {figures/supplementary_qualitative_examples}
                   \caption{
                     %Additional test-set examples from Human3.6m, MPI-INF-3DHP and CMU Panoptic (top to bottom). The examples are selected at the 75, 90 and 99 MPJPE percentiles (left to right).
                     Top to bottom: Additional test set examples from Human3.6m, MPI-INF-3DHP and CMU Panoptic (leftmost person), respectively. The examples from left to right are selected at the 75, 90 and 99 percentiles with respect to the MPJPE between the ground truth (red) and the best-case pose estimate under weak perspective projection (green). The best-case poses under normalized perspective projection (blue) are depicted for the same examples and follow a similar error distribution.
  }
  \label{fig:supplementary_qualitative_examples}
\end{figure*}

\subsection{Best-Case Weak Perspective 3D Estimate}
Recall that the weak perspective projection model allows a perfect depth estimate $\widetilde{Z}_i = Z^\prime_i$.
The mean squared per-joint error for the complete pose estimate is then reduced to
\begin{align}
  \Delta d_2(s)  &= \frac{1}{n} \sum_i \left( X^\prime_i - sx^\prime_i \right )^2 + \left( Y^\prime_i - sy^\prime_i \right )^2 \nonumber \\
                &= \frac{s^2}{n} \left ( \sum_i x_i^{\prime 2} + y_i^{\prime 2}\right ) - \frac{2s}{n} \left ( \sum_i x^\prime_iX^\prime_i + y^\prime_iY^\prime_i\right )  \nonumber \\
  & \; \; \; \;+ \frac{1}{n} \left ( \sum_i X_i^{\prime 2} + Y_i^{\prime 2} \right )b \ ,
\end{align}
where $s$ is the estimated weak perspective scaling factor for the complete pose.
This is again a square function in $s$, with its derivative
\begin{align}
  \Delta d_2'(s)  &= \frac{2s}{n} \left ( \sum_i x_i^{\prime 2} + y_i^{\prime 2}\right ) - \frac{2}{n} \left ( \sum_i x^\prime_iX^\prime_i + y^\prime_iY^\prime_i\right ) \ .
\end{align}
Setting this expression equal to zero yields the optimal scale factor $s^\ast$, with
\begin{align}
	s^* & = \frac{\sum_i X^\prime_ix^\prime_i + Y^\prime_iy^\prime_i}{\sum_i x_i^{\prime 2} + y_i^{\prime 2}} \ .
\end{align}



\section{Qualitative Examples}
We provide additional examples of the best-case 3D human pose estimates under the normalized and weak perspective projection model.
\autoref{fig:supplementary_qualitative_examples} depicts examples from the \emph{Human3.6m} \cite{ionescu14}, \emph{MPI-INF-3DHP} \cite{mehta17} and \emph{CMU Panoptic} \cite{joo15} datasets at different MPJPE percentiles.
The inherent simplifications in the projection models lead to guaranteed and clearly visible discrepancies compared to the 3D ground truth pose.
Note that the largest deviations can be observed for persons that are either clearly off-center (top right, bottom) or very close to the camera (mid), which matches our quantitative results.


\bibliographystyle{ieee}
\bibliography{bibliography}

==> figures/quantitative_results.tex <==
\begin{table*}[]	
	\centering
	\begin{tabularx}{\textwidth}{ l l *{8}{Y}}
		\toprule
		System & Data & Direct. & Discuss & Eat & Greet & Phone & Pose & Purchase & Sit \\
		\midrule
		Drover et al. \cite{drover18} & Synthetic & 48.8 & 51.5 & 41.5 & 57.7 & 49.4 & 54.3 & 48.8 & 50.0 \\
		& Human3.6M & 86.5 & 81.7 & 65.2 & 86.6 & 82.4 & 85.2 & 93.6 & 61.3 \\
		\rule{0pt}{3ex}Ours & Synthetic & 48.8 & 51.5 & 41.5 & 57.7 & 49.4 & 54.3 & 48.8 & 50.0 \\
		& Human3.6M & 86.5 & 81.7 & 65.2 & 86.6 & 82.4 & 85.2 & 93.6 & 61.3 \\
		\bottomrule
		\toprule
		System & Data & SitDown & Smoke & TPhoto & Wait & Walk & WDog & WTog. & \textbf{Avg.}\\
		\midrule
		Drover et al. \cite{drover18} & Synthetic & 64.3 & 51.9 & 64.6 & 57.1 & 54.3 & 57.9 & 53.2 & \textbf{54.8} \\
		& Human3.6M & 82.3 & 73.8 & 93.2 & 85.6 & 78.3 & 80.9 & 82.1 & \textbf{80.4} \\
		\rule{0pt}{3ex}Ours & Synthetic & 48.8 & 51.5 & 41.5 & 57.7 & 49.4 & 54.3 & 48.8 & 50.0 \\
		& Human3.6M & 86.5 & 81.7 & 65.2 & 86.6 & 82.4 & 85.2 & 93.6 & 61.3 \\
		\bottomrule
	\end{tabularx}
	\caption{
		Comparison of the MPJPEs of the replicated system trained and tested with synthetic data and 2D poses from the Human3.6M dataset \cite{ionescu14}. 
		For \cite{drover18} only results with rigid alignment are available, which allows no fair comparison.
		The results were obtained using \textbf{Protocol 2}. The MPJPEs are given in millimeters.
	 }
	\label{tbl:results-quantitative}
	\info[inline]{}
\end{table*}
